An analytic resolution to the competition between Lyman-Werner radiation and metal winds in direct collapse black hole hosts

A near pristine atomic cooling halo close to a star forming galaxy offers a natural pathway for forming massive direct collapse black hole (DCBH) seeds which could be the progenitors of the $z>6$ redshift quasars. The close proximity of the haloes enables a sufficient Lyman-Werner flux to effectively dissociate H$_2$ in the core of the atomic cooling halo. A mild background may also be required to delay star formation in the atomic cooling halo, often attributed to distant background galaxies. In this letter we investigate the impact of metal enrichment from both the background galaxies and the close star forming galaxy under extremely unfavourable conditions such as instantaneous metal mixing. We find that within the time window of DCBH formation, the level of enrichment never exceeds the critical threshold (Z$_{cr} \sim 1 \times 10^{-5} \ \rm Z_{\odot})$, and attains a maximum metallicity of Z $\sim 2 \times 10^{-6} \ \rm Z_{\odot}$. As the system evolves, the metallicity eventually exceeds the critical threshold, long after the DCBH has formed.

==> Makefile <==

USE_BIBTEX=yes
TEX=pdflatex
BIBTEX=bibtex
PDF=dvipdf
all: paper_master.pdf #astroph.pdf

astroph: astroph
# General rules on how to make postscript or PDF versions of a document

paper_master.pdf: paper_master.tex
	$(TEX) paper_master.tex $@
	$(TEX) paper_master.tex $@	
	$(BIBTEX) paper_master
	$(BIBTEX) paper_master
	$(TEX) paper_master.tex $@
	$(BIBTEX) paper_master
	$(TEX) paper_master.tex $@
	$(TEX) paper_master.tex $@

astroph: astroph.tex
	rm -f astroph.pdf
	$(TEX) astroph.tex
	$(TEX) astroph.tex
	$(PDF) astroph.dvi

apj: APJSubmit/apj_regan.tex
	rm -f APJSubmit/apj_regan.dvi APJSubmit/apj_regan.pdf
	cd APJSubmit; $(TEX) apj_regan.tex
	cd APJSubmit; $(TEX) apj_regan.tex
	cd APJSubmit; $(TEX) apj_regan.tex
	cd APJSubmit; dvipdf apj_regan.dvi apj_regan.pdf

mnras: mnras.tex
	$(TEX) mnras.tex $@
	$(TEX) mnras.tex $@	
	$(TEX) mnras.tex $@
	$(PDF) mnras.dvi

.PHONY : clean

clean:
	rm -f *.log *.aux *.out *.dvi *.blg *.toc *.lof *.lot *.tbx \
	 *.fgx *~ paper_master.pdf paper_master.ps *.bbl astroph.pdf

tar:
	tar cvzf submit.tar.gz paper_master.tex paper_master.bbl emulateapj.cls \
	aas_macros.sty apj.bst NEWFIGURES/*.eps

tarastroph:
	tar -cvzf submit.tgz astroph.tex \
	aas_macros.sty FIGURES/ 

tarmnras:
	tar -czvf mnras.tgz mnras.tex aas_macros.sty FIGURES/ BIBTEX/

#filename.ext where the first four characters of filename are the first four 
#characters of your surname and the last four are the current day and month 
#in MMDD format (e.g. smit0531) 
tarapj: clean
	tar -cvzf rega0717.tgz APJSubmit/*.eps APJSubmit/apj_regan.tex

